Synthetic Dataset Generation for Partially Observed Indoor Objects

Learning-based methods for 3D scene reconstruction and object completion require large datasets containing partial scans paired with complete ground-truth geometry. However, acquiring such datasets using real-world scanning systems is costly and time-consuming, particularly when accurate ground truth for occluded regions is required. In this work, we present a virtual scanning framework implemented in Unity for generating realistic synthetic 3D scan datasets. The proposed system simulates the behaviour of real-world scanners using configurable parameters such as scan resolution, measurement range, and distance-dependent noise. Instead of directly sampling mesh surfaces, the framework performs ray-based scanning from virtual viewpoints, enabling realistic modelling of sensor visibility and occlusion effects. In addition, panoramic images captured at the scanner location are used to assign colours to the resulting point clouds. To support scalable dataset creation, the scanner is integrated with a procedural indoor scene generation pipeline that automatically produces diverse room layouts and furniture arrangements. Using this system, we introduce the \textit{V-Scan} dataset, which contains synthetic indoor scans together with object-level partial point clouds, voxel-based occlusion grids, and complete ground-truth geometry. The resulting dataset provides valuable supervision for training and evaluating learning-based methods for scene reconstruction and object completion.

==> old.tex <==
%\saythanks % added 28-02-2014 Markus Englich


%\section{Introduction}
%3D scanning technologies are critical for applications such as object reconstruction, robotic perception, and digital twin creation \cite{vermandere_geometry_2025}. However, collecting high-quality real-world scan data is often time-consuming, expensive, and difficult to reproduce under controlled conditions. To address these challenges, we propose a virtual scanning system developed in Unity that replicates the behaviour of real-world scanners.

% indoor scanned datasets
%synthetic datasets are often created by sampling objects along its surface \cite{de_geyter_automated_2022}. While this is the easiest and fastest way, it leads to unrealistic point distributions and more importantly, points at surfaces that are invisible to a potential scanner. For this reason, there is a need for virtual scans that are taken from set set-up points to ensure realistic occlusions.

% real outdoor driving datasets
%The self driving sector has multiple The KITTI dataset  \cite{geiger_are_2012} contains 389 stereo and optical flow image pairs, stereo visual odometry sequences of 39.2 km length, and more than 200k 3D object annotations captured in cluttered scenarios.

% real indoor datasets
%Datasets of indoor environments have already been made like Matterport3D\cite{chang_matterport3d_2017} and Scannet++ \cite{yeshwanth_scannet_2023}. However, since they originate from real environments, they lack any actual ground truth data.

% synthetic indoor datasets
%ShapeNet \cite{chang_shapenet_2015} on the other hand is a fully synthetic dataset of ** objects over ** classes. Since they are synthetic, simply sampling them also results in extra points inside the object due to the extra faces present of all the sub-meshes.

% existing virtual scanners
%Existing virtual laser scanners focus on the educational aspect of learning how to best employ a laser scanner in the field \cite{popovas_virtual_2021}. 
%Other implementations focus on aerial laser scanning from a virtual plane. \cite{winiwarter_virtual_2022}

% occlusion detection
%The detection of what areas are occluded from a scanner during capture (e.g. occlusion detection) can greatly improve the completion results for objects. Other fields like robotics \cite{zhu_occlusion_2020} already use this method to estimate the safe areas to navigate

% The main contribution
%The main contributions of this work are twofold:
%\begin{itemize}
%    \item Creating an easy-to-use plug-and-play Virtual scanner for the Unity game engine that can be placed in any virtual scene to create a virtual 3D scan.
%    \item Calculating full-scene and per-object occlusion voxel grids for downstream completion network inputs.
%    \item Providing a dataset of 100s partially scanned 3D object with proper ground truth.
%\end{itemize}
%The virtual scanner and accompanying dataset will enable further and more thorough training of SOA object completion models.

\section{Introduction}

Three-dimensional (3D) scanning technologies play a crucial role in fields such as object reconstruction, robotic perception, and digital twin generation \cite{vermandere_geometry_2025}. However, acquiring large amounts of high-quality real-world scan data for training machine learning (ML) models is often time-consuming and costly. To address these challenges, we propose a virtual scanning framework developed in Unity that replicates the behaviour and characteristics of real-world scanners to create a synthetic dataset of realistically scanned environments.

Synthetic 3D datasets are frequently generated by directly sampling points on the surfaces of 3D objects \cite{de_geyter_automated_2022}. Large-scale repositories such as \textit{ShapeNet} \cite{chang_shapenet_2015} provide extensive collections of 3D object models across hundreds of categories. Although this approach is fast and straightforward, it produces unrealistic point distributions and includes points on surfaces that would be invisible to a real scanner. As a result, such datasets fail to accurately model occlusions or realistic acquisition noise. A more realistic alternative is to simulate scans from defined viewpoints, thereby ensuring that occlusions and sensor limitations are faithfully reproduced.

In the autonomous driving domain, datasets such as \textit{KITTI} \cite{geiger_are_2012} provide a large collection of real-world stereo images, optical flow data, and 3D annotations captured in complex outdoor environments. Similarly, for indoor settings, datasets like \textit{Matterport3D} \cite{chang_matterport3d_2017} and \textit{ScanNet++} \cite{yeshwanth_scannet_2023} offer high-quality RGB-D scans of real interiors.  
While these datasets are invaluable, they lack complete ground truth geometry. This limitation constrains their usefulness for tasks that require accurate, fully known reference data, such as training ML models for geometric completion.

Existing virtual laser scanner tools primarily focus on educational or domain-specific applications. For example, \cite{popovas_virtual_2021} present a simulator designed for training users on laser scanning techniques, while \cite{winiwarter_virtual_2022} focus on aerial LiDAR scanning from virtual aircraft. These implementations, though useful, are not intended for large-scale synthetic dataset generation or occlusion-aware data production.

Accurately modeling occlusions is essential for many downstream applications. Occlusion detection helps identify regions of a scene that are invisible from a given scanner position and can substantially improve object completion and reconstruction tasks. In robotics, similar techniques are employed for visibility reasoning and safe navigation planning \cite{zhu_occlusion_2020}. Integrating such mechanisms into a virtual scanning system allows for the generation of realistic partial observations along with ground-truth visibility maps.

The main contributions of this work are as follows:
\begin{itemize}
    \item \textbf{Virtual Scanner for Unity:} We introduce an easy-to-use, plug-and-play virtual scanner module for the Unity game engine. It can be placed within any virtual environment to produce realistic 3D scans from arbitrary viewpoints.
    \item \textbf{Occlusion Voxel Grids:} We compute both full-scene and per-object occlusion voxel grids to provide detailed visibility information, enabling their direct use as inputs for completion and reconstruction networks.
    \item \textbf{Synthetic Dataset:} We release a dataset comprising hundreds of partially scanned 3D objects, each paired with corresponding complete ground-truth models for benchmarking and training state-of-the-art completion methods.
\end{itemize}

Overall, the proposed system bridges the gap between simplistic surface sampling and costly real-world data collection. By combining photorealistic rendering with physically plausible scan simulation, our framework enables the creation of high-quality synthetic datasets suitable for training, evaluation, and benchmarking of 3D perception algorithms.


\section{Methodology}

In this section, the creation of the Virtual scanner is discussed along with the object isolation and occlusion calculation.


\subsection{Scanner Setup}
To replicate the operation of a physical 3D scanner in a digital environment, a set of parameters is defined to emulate real-world scanning behaviours. Several presets are also provided to approximate popular commercial scanner types. The main parameters are:

\begin{itemize}
    \item \textbf{Scan density} ($d_s$, in mm/10m)
    \item \textbf{Scan range} ($r_{\max}$, in m)
    \item \textbf{Vertical scan range} ($\theta_{\max}$, in degrees)
    \item \textbf{System error} ($\varepsilon_s$, in mm)
    \item \textbf{Distance error} ($\varepsilon_d$, in \%)
\end{itemize}

These parameters enable the simulation to mimic different scanner characteristics, such as resolution, measurement precision, and angular coverage. Figure \ref{fig:scanner_scene} shows the setup of the scanner in a Unity scene.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/virtual scanner screenshot.png}
    \caption{A screenshot of the virtual scanner setup, where the scanner is placed in a scene (left) and the parameters are visible on the right.}
    \label{fig:scanner_scene}
\end{figure}

\subsection{Creating Scan Vectors}
The scanning process begins with defining the desired resolution, from which a spherical array of scan vectors is generated. Each vector represents a single scanning ray. The array is formed by distributing vectors over horizontal disks stacked along the vertical axis, beginning from a minimal elevation angle $\theta_{\min}$ to simulate the blind zone beneath the sensor. Although this method differs from the sequential vertical scanning typical of many physical systems, it produces a more uniform and computationally efficient sampling pattern for synthetic data generation.

%Let $\phi$ denote the azimuthal angle and $\theta$ the polar (vertical) angle. For each pair $(\phi_i, \theta_j)$, a direction vector $\mathbf{v}_{ij}$ is defined in Cartesian coordinates as:

%\begin{equation}
%\mathbf{v}_{ij} =
%\begin{bmatrix}
%\cos\theta_j \cos\phi_i \\
%\cos\theta_j \sin\phi_i \\
%\sin\theta_j
%\end{bmatrix},
%\end{equation}

%where $\phi_i \in [0, 2\pi)$ and $\theta_j \in [\theta_{\min}, \theta_{\max}]$.  
%

\subsection{Scanning Process}
During the scanning phase, a ray is cast along each direction vector $\mathbf{v}_{ij}$ from the scanner origin $\mathbf{o}$ until it intersects a surface in the scene. The intersection point $\mathbf{p}_{ij}$ is given by:

\begin{equation}
\mathbf{p}_{ij} = \mathbf{o} + r_{ij}\mathbf{v}_{ij},
\end{equation}

where $r_{ij}$ is the measured distance to the surface along that ray.  
To simulate sensor inaccuracies, random noise is added to the measured distance:

\begin{equation}
r_{ij}' = r_{ij} + \mathcal{N}(0, \varepsilon_s) + r_{ij}\varepsilon_d,
\end{equation}

where $\mathcal{N}(0, \varepsilon_s)$ represents Gaussian noise with zero mean and standard deviation $\varepsilon_s$, and $\varepsilon_d$ models proportional distance error.  
If no intersection occurs within the maximum range $r_{\max}$, no point is recorded. The final point is stored at position $\mathbf{p}_{ij}' = \mathbf{o} + r_{ij}'\mathbf{v}_{ij}$, forming part of the synthetic point cloud.

\subsection{Point Colouring}
To assign realistic colour values, a $360^{\circ}$ panoramic image is captured from the scanner’s position. This allows ambient lighting and shading conditions in the virtual scene to influence the point colours, mimicking real-world acquisition.

Each point $\mathbf{p}_{ij}'$ is coloured by converting its angular coordinates $(\phi_i, \theta_j)$ into UV texture coordinates for sampling the spherical image:

\begin{equation}
u = \frac{\phi_i}{2\pi}, \qquad v = \frac{\theta_j - \theta_{\min}}{\theta_{\max} - \theta_{\min}}.
\end{equation}

The corresponding pixel colour at $(u, v)$ is then assigned to the scanned point and the whole point cloud can be exported to a number of formats.
%This approach ensures that the final colored point cloud accurately captures both the geometric structure and the lighting conditions of the simulated environment.

\subsection{Object Scanning and Occlusion Calculation}

To enable per-object analysis and ground-truth generation, each object in the 3D scene is first isolated based on its spatial extent. Since objects are represented as separate entities in the virtual environment, their \textit{oriented bounding boxes} (OBBs) can be computed directly from their geometry. These bounding boxes define spatial regions within which all corresponding scan points must reside. The boundaries of each region can be further expanded or contracted by a user-defined offset.
 
Within each object’s bounding box, an \textit{occlusion grid} is constructed to quantify the visibility of individual voxels from the scanner’s origin. Each voxel is evaluated by casting a ray toward its centre; if the ray intersects another surface before reaching the voxel, the voxel is marked as occluded.
Each occlusion grid is exported together with the corresponding partial object scan. These paired outputs provide both the incomplete point cloud (as captured by the simulated scan) and its corresponding visibility map, enabling their use as supervised inputs for object completion and reconstruction networks.



%%%generated

%\subsection{Object Scanning and occlusion calculation}

% isolating each object
%We can isolate all the points of an object.
%Each object is separate in the 3D scene, by getting the oriented bounding box, a region can be defined where all the points must be inside of. this region can be offset by the user. Within each of these object boundingboxes, an occlusion grid is calculated based on the visibility of the voxel to the scanners origin. This occlusion grid can then be exported, together with the partial object scan to use in object completion networks as an input.


\section{Dataset}
% we compare the resulting virtual scans of the environments to 
The results from the Virtual scanner are consolidated into a dataset, these will be expanded upon and made available in the full paper. A sample can be seen in Figure \ref{fig:cloudcompare}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/virtual scanner screenshot_2.png}
    \caption{The resulting coloured 3D pointcloud from a virtual scan.}
    \label{fig:cloudcompare}
\end{figure}

\section{Conclusion}

In this work, we presented a virtual 3D scanning framework implemented in Unity that accurately replicates the behavior of real-world scanners. By simulating realistic scanning parameters, measurement noise, and occlusion effects, the system enables the generation of high-fidelity synthetic datasets suitable for training and evaluating 3D perception algorithms. 

The framework supports both scene-level and object-level scanning, providing not only partial point clouds but also corresponding occlusion grids and complete ground-truth geometry. These outputs facilitate the development of data-driven object completion and reconstruction methods under realistic observation constraints.

The full paper will dive deeper in the voxel occupancy calculations, the object isolation and showcase the full dataset.

